MechStyle: Augmenting Generative AI with Mechanical Simulation to Create Stylized and Structurally Viable 3D Models

Recent developments in Generative AI enable creators to stylize 3D models based on text prompts. These methods change the 3D model geometry, which can compromise the model's structural integrity once fabricated. We present MechStyle, a system that enables creators to stylize 3D printable models while preserving their structural integrity. MechStyle accomplishes this by augmenting the Generative AI-based stylization process with feedback from a Finite Element Analysis (FEA) simulation. As the stylization process modifies the geometry to approximate the desired style, feedback from the FEA simulation reduces modifications to regions with increased stress. We evaluate the effectiveness of FEA simulation feedback in the augmented stylization process by comparing three stylization control strategies. We also investigate the time efficiency of our approach by comparing three adaptive scheduling strategies. Finally, we demonstrate MechStyle's user interface that allows users to generate stylized and structurally viable 3D models and provide five example applications.

==> Sections/04_mechanical_property_backup.tex <==
\section{Simulation Augmented 3D Stylization}

MechStyle is a system that integrates mechanical simulation into the 3D model stylization process to preserve a 3D model's structural integrity while manipulating the model according to the desired style. As the stylization process iterates, MechStyle simulates intermediate stylized versions of the model to identify local regions where the stress has increased. For those regions, MechStyle reduces stylization in subsequent iterations.

We investigate two specific challenges to accomplish mechanical simulation into the stylization process. First, we provide a method to incorporate the stress results from a simulation of an intermediate version of the model into the generative AI stylization process that modifies the model geometry. Second, since simulation is computationally intensive, we examine different scheduling approaches that determine when the simulation should be executed in the stylization process to preserve structural integrity. 

We next describe the model architecture we set up to incorporate simulation results into the stylization process and then describe how we address the first challenge by developing three differing stylization control strategies and the second by developing three different adaptive scheduling strategies for the simulation.

% In this section, we describe how we modify the stylization model architecture and incorporate simulation results into the process. Given that simulating is a computationally expensive process, we also describe a method to run simulations efficiently. 

\subsection{Model Architecture Integrating Stylization and Simulation}
\label{section:system-simulation}
% \stefanie{we need some method to map the local stress values from the mechanical simulation to the vertices from the stylization}
% \faraz{Make the title to have a sense of both}
% \stefanie{Shared Weights/Data Formats}

We set up our model architecture as a dual-network with two components: (1) the stylization module, and (2) the simulation module. The stylization module iteratively modifies the geometry. The simulation module tracks changes in stress on the model resulting from the modified geometry. Stylization occurs in every iteration, while simulation is run at specific intervals. When stress increases in the model at a particular region, the simulation module identifies it. It communicates it to the stylization module as a \textit{mask} over regions of high stress. The stylization module then reduces the number of modifications to these areas in subsequent iterations. By reducing local modification, the following iterations preserve the stress/strain characteristics over these regions.  Thus, these two modules work in tandem, iteratively stylizing the model while controlling for the impact on structural integrity.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/mechstyle-system.png}
    \caption{System Architecture: }
    \label{fig:system_figure}
\end{figure}

\subsubsection{Stylization Method} 
We define 3D model as an input mesh  $M$ with vertices in Cartesian coordinate $\mathbb{V} \in \mathbb{R}^{nx3}$ connected by faces $\mathbb{F} \in \{1,...n\}^{mx3}$ with color channels $\mathbb{C} \in \mathbb{R}^{nx3}$ corresponding to R,G,B colors. We use the X-Mesh~\cite{x_mesh} model architecture for stylization, which takes a text prompt from the user and iteratively displaces each model vertice and modifies their color channels to conform to the text prompt. Vertices are shifted along their normal to the mesh surface. The set $\mathbb{D} = \{d_v \forall v \in \mathbb{V}\}$ defines the distance along each normal the vertex will move in a given iteration. That is, stylization shifts each vertex $v$ by a distance of $d_v$ along the normal of $v$ relative to the mesh. This forms a modified 3D model geometry. The color of the model is shifted with similar displacements of the color channel $\mathbb{C}$. We run this process for 200 iterations, which has been shown to converge on a solution across a variety of models and styles~\cite{x_mesh}. This results in a stylized model $M_s$.



\subsubsection{Mechanical Simulation Method}
Our choice of simulation was informed by two constraints: the mechanical simulation should be able to support complex geometries and be computationally efficient to simulate many intermediate iterations of the stylization. We, therefore, use a solid FEA-based method based on tetrahedral elements using a hyperelastic neo-hookean constitutive model~\cite{smith2018stable}. We implemented this using NVIDIA Warp~\cite{warp2022}, a Python framework for developing differentiable GPU-accelerated high-performance simulations. This simulation is material-specific and is initialized using a given material's Lamé parameters. The Lamé parameters, denoted as $\lambda$ and $\mu$, are material constants used in the field of elasticity and solid mechanics. These can be calculated using a material's Young's Modulus (E) and Poisson's ratio ($\nu$). For our paper, we focus on the widely used material PLA for 3D printing. Additional materials can be added by changing the Lamé parameters provided to the simulation. 

% \begin{equation}
%     \lambda = \frac{E \nu}{(1 + \nu)(1 - 2\nu)}\\
% \end{equation}

% \begin{equation}
%     \mu = \frac{E}{2(1 + \nu)}
% \end{equation}

% We simulate the 3D model as a deformable 3D solids and calculate the local internal strain and stress values due to the forces exerted on the objects. 
% \vspace{5pt}
% \noindent\textbf{Mechanical Simulation Setup:} 

FEA analysis of 3D models is traditionally done under well-specified boundary conditions. These conditions are set by specifying the locations of loads (forces) on the model and their magnitude. Since the loads are specific to the model and its use case, engineers typically set them manually before simulation. However, since our target users are non-experts who may not be able to identify the load requirements of a model apriori, we cannot rely on these inputs in MechStyle. Alternatively, Langlois et al.~\cite{stochastic_structural_analysis} proposed a model- and use-case agnostic stochastic FEA simulation technique that includes simulating a model under a Drop Test scenario. They simulate the model dropping on a hard surface from a random height and generate stress distributions on the model using the forces contracted on the model during the simulation. We use a similar approach where we simulate the model dropping from a specific height on a hard surface. We store the per-element von Mises stress values, a standard metric used in continuum mechanics \cite{fill this in}\hl{REF}. We extract the maximum stress at any time in the simulation for every element on the mesh. This highlights the model's most vulnerable points.  

% \faraz{Notes: 
% Warp is a programming language, and we use the FEM model. We use a CUDA accelerated FEM implementation. Explicit solver for FEM instead of a Generative solver}



\subsection{Constraining Local Stylization via Masking}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/masking_strategies-two-col.png}
    \caption{Masking Strategies}
    \label{fig:masking_strategies}
\end{figure*}

As discussed above, stylization progresses by iteratively modifying a model with small displacements of its vertices and changes in their color. These changes are done gradually, with each vertex changing the model by <1\% of the model size after each iteration of stylization~\cite{x_mesh}. Thus, we can identify regions where local stresses are increasing by simulating an intermediate version of the 3D model as it is being stylized. After identifying regions where stress increases, we can locally reduce stylization to prevent further stylization's impact on the structural integrity of the model. Next, we present our method to identify local regions with increased stress and then present different stylization control strategies that modify subsequent local stylization in areas with increased stress. 


\subsubsection{Simulation-Informed Stylization via Masking:} 
We first simulate the original un-stylized model $M_0$ to calculate the set of maximum local von Mises stress values on each vertex in the model, $\mathbb{S}_0=\{s_{v_0} \forall v_0 \in \mathbb{V}_{M_0}\}$.
% for each vertex across frames $S \in \mathbb{R}^n$, where $n$ is the number of vertices.
For a specific iteration $i$ of the stylization progresses, $M_0$ is modified to create an intermediate geometry $M_{i}$. We simulate this intermediate geometry of $M_i$ to extract the stress distribution $\mathbb{S}_{i}$. To compare the local stress changes from the original model to the stylized model, we calculate a normalized stress vector $\mathbb{S}_{norm}(i)$ (\autoref{eq:S_norm}) by dividing this updated stress distribution $\mathbb{S}_i$ by that of the original model $\mathbb{S}_0$.

\begin{equation}\label{eq:s_norm}
    s_{norm}(v_i) = \frac{s_{v_i}}{s_{v_0}}
\end{equation}
\begin{equation}\label{eq:S_norm}
    \mathbb{S}_{norm}(i) = \{s_{norm}(v_i) \forall v_i \in \mathbb{V}_{M_i}\}
\end{equation}

% \begin{equation}
%     S^{norm} = \frac{S^{i}}{S}
% \end{equation}


These normalized stress values help to identify vertices where the stylization process has increased stress on the model. For a vertex $v_i$ on the model $M_i$ produced by the $i$th iteration of stylization, the normalized stress value is $s_{norm}(v_i)$ (\autoref{eq:s_norm}). When $s_{norm}(v_i) > 1$, the stress on the model $M_i$ at that vertex has increased since the original model. Conversely, when $s_{norm}(v_i) \leq 1$, the stress was reduced or remained the same compared to the original model. Thus, these values can be used to identify vertices where stress has increased and then reduce subsequent stylization at those vertices. Recall that stylization iteratively modifies the model vertices $V$ by the displacement $\mathbb{D}$. MechStyle modifies this displacement by applying a mask to each displacement of each vertex $v$. The masking function uses the normalized stress distribution to locally reduce or freeze geometry displacement where it is causing added strain. This produces the masked displacement set $\mathbb{D}_{norm}$ (see \label{eq:d_norm}).
% For this, we first apply a ReLU function on $S^{norm}$. 
% \begin{equation}
%     S^{relu} = max(1, S^{norm})
% \end{equation}

% $S^{relu}_j = 1$ for vertices where stress is lower or equal to the original, and higher for locations where the stress has increased.

% We can control stylization differently by utilizing different strategies. We evaluate different masking strategies and their impact on the stylization and structural results.

\begin{equation} \label{eq:d_norm}
    \mathbb{D}_{norm} = \{d_v * mask_v \forall v \in \mathbb{V}_M\}
    % d_{norm} = d * mask
\end{equation}

We do not normalize the color modification values since they do not impact structural properties. In the next section, we describe three stylization control strategies that apply the mask with $\mathbb{S}_{norm}$ in different ways to reduce stylization in regions with increased stresses while staying close to the user's stylization prompt.

\subsubsection{Stylization Control Strategies:}
\label{sec:masking-strategies}
We developed three different stylization control strategies that reduce stylization by different amounts in regions with increased local stresses. The first strategy linearly reduces per-vertex displacement according to the increase in stress. The second approach exponentially reduces the per-vertex stylization. The third approach stops the stylization completely in those regions.  

\paragraph{Linearly Weighted Stylization:} For the linearly weighted stylization, we normalize stylization by a factor related to how much the stress has increased compared to the corresponding local stress in the original model. This approach modulates the displacement values, creating more subtle adjustments during stylization in the model regions with increased stress. This allows for more controlled stylization with reduced impact on the stress in that region. \autoref{eq:linear} shows the linear masking function for a vertex in the model $M_i$.
 
\begin{equation}\label{eq:linear}
    mask_{v_i}=\begin{cases}
            \frac{1}{s_{norm}(v_i)} & \text{if } s_{norm}(v_i) > 1\\
             1 & \text{if } s_{norm}(v_i) \leq 1 
        \end{cases}
\end{equation}
% \begin{equation}
%     mask_i=\begin{cases}
%             1 / S^{norm}_i & \text{if } {S}^{norm}_i > 1\\
%              1 & \text{if } {S}^{norm}_i \leq 1 
%         \end{cases}, \quad \forall i \in V
% \end{equation}



\paragraph{Exponentially Weighted Stylization:} For the exponentially weighted stylization, we exponentially reduce the stylization in areas with increased stress. This technique reduces stylization more aggressively compared to the Linearly Weighted approach. To compute the mask, we calculate the negative exponent of $(S^{\text{norm}}_i - 1)$, which results in a value between 0 and 1 for $S^{\text{norm}}_i > 1$. This means the resulting stylization is exponentially smaller as the stress increases. \autoref{eq:exponential} show the exponential masking function for a given vertex. 

\begin{equation} \label{eq:exponential}
    mask_{v_i} = \begin{cases}
    e^{-(s_{norm}(v_i) - 1)} & \text{if } s_{norm}(v_i) > 1\\
    1 & \text{if } s_{norm}(v_i) \leq 1 
    \end{cases}
\end{equation}

% \begin{equation}
%     mask_i = \begin{cases}
%     e^{-(S^{\text{norm}}_i - 1)} & \text{if } S^{\text{norm}}_i > 1\\
%     1 & \text{if } {S}^{norm}_i \leq 1 
%     \end{cases}, \quad \forall i \in V
% \end{equation}

\paragraph{Selectively Frozen Stylization:} For the selectively-frozen stylization technique, once the local stress in a region increases beyond the corresponding local stress in the original model, we set the displacement matrix to 0 for these vertices, resulting in no more stylization of that region. This method is similar to that employed in Style2Fab~\cite{faruqi2023style2fab} where stylization is frozen in functional segments of the model.


\begin{equation}\label{eq:frozen}
    mask_{v_i}=\begin{cases}
            0& \text{if } s_{norm}(v_i) > 1\\
             1& \text{if } s_{norm}(v_i) \leq  1 
        \end{cases}
\end{equation}
% \begin{equation}
%     mask_i=\begin{cases}
%             0& \text{if } S^{norm}_i > 1\\
%              1& \text{if } S^{norm}_i \leq  1 
%         \end{cases}\\
%         \quad \forall i \in V
% \end{equation}


In summary, we control the per-vertex stylization in areas with increased stresses by creating a mask based on the simulation results. Then, we normalize the displacement vector $\mathbb{D}$ before applying it to the model $M_i$. We compare these different stylization control strategies in our technical evaluation, which demonstrates a trade-off between how closely the desired style was approximated (i.e., style-loss) and how well the model's original structural integrity was preserved (i.e., structural-loss).
 


% During the simulation, we calculate the maximum local Von Mises stress ~\faraz{get paper}. We then output the stress values in the form of a matrix, where each stress value in the matrix corresponds to a vertex in the model. We then normalize the matrix that contains the stress values with the matrix that contains the stress values of the original unmodified 3D model. This new matrix has the same shape as the vertices array of the model being stylized. Thus, this can be used as a mask to normalize any subsequent manipulations to the model by dividing the displacement values output by the generative AI. This updated displacement matrix has reduced stylization values for the high-stress areas and the same displacement for other areas. With this method, the areas that are under high local stress will be manipulated minimally in the consequent stylization iterations, while the other sections will be stylized as needed. 

\subsection{Adaptive Scheduling of FEA Simulation}
\label{sec:scheduling-strategies}
% \vspace{5pt}
% \noindent\textbf{When to simulate}:

Normalizing the displacement of vertices at each stylization step with a mask generated based on local simulated stress changes preserves structural integrity during the stylization process. However, another important factor to consider for this integration is the total run-time of the combined system. FEA simulations are traditionally computationally intensive, and even though we leverage a GPU-accelerated simulation, it is computationally prohibitive to run simulations at each iteration step. In this section, we discuss different strategies to efficiently run simulations during stylization.  

\subsubsection{Differences in Stylization and Simulation Times:}
Ideally, FEA simulations would assess stress changes after each iteration of stylization. However, the run-time for a single FEA simulation is significantly more than that of one stylization iteration. Across the 30 models from our formative study dataset, one iteration of stylization with any style takes \hl{XX} seconds, while the FEA simulation of the same models took an average of \hl{YY} minutes. Since stylization runs for 200 iterations before convergence, simulating after each iteration increases the average run-time to \hl{ZZ} minutes. Therefore, running FEA simulations at the same granularity as stylization is computationally prohibitive. Notably, simulation must be completed across a whole model, even if only a small region is displaced in an iteration. This is because localized changes in geometry may have global effects on the model, which will only reveal themselves in a full simulation. For example, suppose that stylization reduces the thickness in one portion of a phone stand. While this section may remain structurally sound, the weight placed in a different region by a phone or tablet may reveal strain that would snap the holder at this thinned region. While there may be model-specific strategies for more efficiently simulating these effects, there are no model-agnostic simulation strategies that require only localized geometry \cite{needed}. 

However, two features of the stylization process suggest that an adaptive strategy of running simulations at specific instances during the stylization might suffice. Firstly, stylization proceeds iteratively, where the magnitude of $|d_v|$ for all vertices is less than 1\% of the model size~\cite{x_mesh}. These subtle changes suggest that running FEA simulations at the same granularity as stylization is unnecessary.  Secondly, our formative study showed that different styles impact different 3D models differently and that different models are impacted differently by the same style. Thus, a stylization-agnostic and model-agnostic simulation technique could either be excessive or deficient depending on context. 

% By investigating geometry changes of stylization per iteration, we found that simulation after each iteration does not yield proportionately valuable insights into the structural integrity of the model at every iteration step. The reason for this is that stylization only creates minimal model modifications. Using the formative study dataset, we compared the displacement amount after each iteration to the model's size of the previous iteration and found that the displacement was at maximum 1\% of the original model size. 

% Finally, we found that when to run mechanical simulation in the stylization process cannot be accomplished with the same step size because different styles impact models differently, and different models are impacted by different amounts by the same style (see Formative Study). Thus, a stylization-agnostic and model-agnostic technique of simulation could either be excessive or deficient. 

% \vspace{5pt}
% \noindent\textbf{Adaptive Scheduling Strategies:} 
To develop an adaptive method to determine which iterations of stylization require simulation, we explored three different scheduling strategies. The first is based on temporally distributing simulation, which simulates more frequently in the initial stages of stylization to preserve weak areas with increased stress. The second approach correlates the iterative geometry change with the local 3D model thickness and simulates if the relative geometric change exceeds the local thickness-informed threshold. Finally, the third approach correlates the geometric change from stylization to the local normalized stress, triggering a simulation when geometric change exceeds the local stress-informed threshold. 


% , where we use a uniform temporal distribution, ensuring consistent monitoring at equidistant points during the stylization process. 

\paragraph{Non-Linear Temporal Scheduling:}
This technique employs a non-linear scheduling interval that increases as stylization progresses. The reason we use this strategy is that stylization makes larger geometry changes at early iterations, but as stylization converges to the desired style, geometry changes become more subtle. Moreover, displacements across iterations accumulate over iterations throughout the stylization. Thus, simulating more often early in the process allows us to capture stress changes related to those early geometry changes. Some examples of a non-even scheduling strategy are quadratic or exponential scheduling over the stylization process.

% This approach optimizes computational resources by allocating them more heavily toward the start of the stylization process.

\paragraph{Geometry-Based Scheduling:}
This scheduling strategy determines when to run the FEA simulation based on the cumulative displacement of vertices with respect to the local model thickness. This approach is motivated by the fact that models with thin segments are more impacted by stylization than thicker geometries. Thus, even small vertex displacements on thin geometries influence the structural integrity of the model. We track cumulative displacement at all vertices across iterations, and simulations are triggered when displacement surpasses a threshold based on the model thickness. This method ensures that simulations are conducted in direct response to the stylization's impact on the model rather than at predetermined intervals. This scheduling method is more responsive to the mesh modification.

% \stefanie{This threshold progressively increases with a factor, allowing for more stylization iterations before simulating again. }

\paragraph{Stress-Based Scheduling:}
This technique refines the geometric tracking approach defined above by incorporating an initial analysis of regions with high stress, focusing subsequent geometric change tracking on these areas. This method uses the original model's stress distribution to identify regions with higher stresses and assigns proportional thresholds for geometric changes. The vertices associated with the maximum stress are assigned lower thresholds, while regions with lower stresses are assigned greater thresholds, allowing for more stylization before triggering a simulation. Simulations are triggered when displacements for vertices exceed their specific thresholds. The resulting stress distribution from the simulation is used to update the mask, reducing the stylization on these vertices. By monitoring changes in weaker areas more closely, this method ensures that simulations are prioritized based on the potential risk to the model’s structural viability while reducing the potential of unnecessary simulations, enhancing the system's efficiency.

In summary, our goal was to develop a simulation scheduling strategy method that adaptively resolves when to simulate an intermediate step of the stylization process to minimize run-time while ensuring structural integrity. We present three different scheduling strategies and evaluate them for structural changes and run-time.  

% This threshold array (size equal to number of vertices) is progressively increased with a factor of two after each simulation, allowing for more stylization iterations after the mask update.


% \stefanie{one idea might be to fully stylize the model, then run mechanical simulation, and then only look at those parts again that had some problem. however, we cannot just use the local area to run in mechanical simulation, we always have to test the whole model, so there is no time saving on the mechanical side. but we could save a little bit of time by locally restylizing rather than globally. but that's not significant since MechE simulation is the real time sucker.}


% \stefanie{another idea is to run one mechanical simulation on the original model using a worse-case-style with maximum vertex offset (and we have to figure out what a worst-case style is). The user can then select from the slider if they want to stylize weak regions or not, and we know what weak regions are because we already have information from the worst case style simulation. Next, the user can look at the stylization iteration slider to check if they like how the style looks even when local weak regions where not styled or only a little styled. This can be done in real-time after only waiting for stylization to finish (8 minutes). While the user can explore the stylization result, we parallel process the actual mechanical simulation result for each style iteration. This takes longer (3 min per style iteration), and will become available in the UI/slider later. }

% \stefanie{Probably the final idea: Based on a dataset of similar models that underwent some geometry modification and then had some mechanical simulation results, we know that if we change our model by a certain amount (offsetting vertices), it is likely we have to resimulate because the other similar model required simulation to figure out new weak regions. The hope is that this mean that once we finished stylizing the weak regions up to a certain threshold/level, we may not need mechanical simulation anymore because the main model geometry will not have enough geometry change to require simulation. Convergence. Stylization has a lot of impact at the beginning, but the longer it runs the smaller the modifications are, i.e. it converges. Because of that, we have to run mechanical simulation more often at the beginning but not that much at the end.}



% \stefanie{Impact of Material Choice on Simulation Time. Impact of Vertex numbers of Simulation Time. Calculating Van Mises only on max force rather than on each step. Maybe Worst Case Stylze first to preprocess model with mechanical results.}


% Thus, this matrix can be used 


%  We normalize the simulation result with the maximal stress from the original model, and then use this as a weight matrix to normalize the subsequent manipulations on the model.
 

% This is important since X-Mesh utilizes a similar matrix to compute the iterative manipulation on the geometry for the model. 

% With this weighted matrix, the areas that are under high local stress will be manipulated minimally in the consequent stylization iterations, while the other sections will be stylized as needed. 




% This system design required to have a gradient-based simulation method, similar to the aesthetic manipulation method. This would allow the simulation module to send feedback to the stylization module, and allow them to work in tandem. 

% The model is represented as a matrix, where each row is a vertex and the columns represent the X, Y and Z positions, followed by the RGB colors. 

% This matrix is updated with each iteration, with the displacement matrix containing the amount of manipulation for each vertex. As the stylization progresses, X-Mesh reduces the CLIP distance between the original model rendering and the desired style by makes iterative changes on the model. 

% considers a 3D model as a collection of vertices with color channels (RGB), where the vertices can be displaced along their normals, and the color channels can range between 0 to 255. 



% To stylize 3D models, we leverage the X-Mesh~\cite{x_mesh} system. X-Mesh takes snapshots of the 3D model from multiple views, and uses CLIP~\cite{radford2021learning} representation to compare against the style given by the user in form of text. The system considers a 3D model as a collection of vertices with color channels (RGB), where the vertices can be displaced along their normals, and the color channels can range between 0 to 255.

% The model is represented as a matrix, where each row is a vertex and the columns represent the X, Y and Z positions, followed by the RGB colors. This matrix is updated with each iteration, with the displacement matrix containing the amount of manipulation for each vertex. As the stylization progresses, X-Mesh reduces the CLIP distance between the original model rendering and the desired style by makes iterative changes on the model. 

% This system design required to have a gradient-based simulation method, similar to the aesthetic manipulation method. This would allow the simulation module to send feedback to the stylization module, and allow them to work in tandem. 

% \faraz{Add a figure which has the two systems talking to each other}






% reducing the gap between this model and the desired style.






==> Sections/09_discussion_extended.tex <==
\section{Discussion and Limitations}
MechStyle is a system that compromises between the benefits and limitations of two approaches to 3D modeling and fabrication. The traditional method of computational design enables an expert modeler (e.g., a mechanical engineer) to craft geometry that serves a particular purpose. In this model, simulation is a tool the expert can use on-demand to evaluate their model. In this use case, the expert can set up a simulation to match the exact use cases they are designing for. Based on the results of a simulation, the expert modifies the geometry to improve mechanical viability while taking other factors under consideration (e.g., aesthetics, use cases, hardware limitations). Since these experts often spend substantial time between iterations, it is acceptable for simulation to be computationally complex and not run in real time. This traditional CAD pipeline assumes a lone modeler with expertise and awareness of the context of their model will be used and an abundance of time to review and iterate on their design.

Generative AI provides an emerging method for creating fabricatable 3D models. Unlike the traditional approach, these methods require little more than a text prompt and a model as a starting point. This makes them particularly well suited to novice modelers who do not have the expertise to effectively use traditional tools. However, neither the AI nor the user are domain experts. If a novice modeler is reusing an existing model--crafted by an expert with traditional tools--then both AI cannot rely on the novice's analysis of the model. A novice modeler is unlikely to be able to specify the load requirements of the model, which parts of the geometry are critical to its integrity, and which can be freely stylized. Under this emerging method of 3D modeling, we must develop systems that reconsider the limitations of existing mechanical simulation methods. 

In developing MechStyle, we make three critical assumptions about these novice modeling contexts to find a tractable solution to include simulation in a generative AI stylization process. Each of these assumptions limits the capabilities of the system and reflects opportunities for future work. First, we assume that modelers provide a working original model that satisfies all of their requirements in the real world. Second, we assume a direct correlation between simulated stress and strain and the mechanical of a model post-fabrication. Third, we assume that a drop-test is a sufficient approximation of the stresses and strains put on a model in regular use. While our evaluation and demonstrations show that these assumptions hold under a variety of scenarios, there are likely many scenarios where these will not suffice, and MechStyle may produce broken models. 

\subsection{Modifying vs Generating Models}
MechStyle works by preserving the mechanical properties of the original model. If that original model meets the user's requirements, this will preserve those critical properties. However, if a user inputs a 3D model that is not mechanically viable, the system may preserve the pieces of the model that make it mechanically unsound. Indeed, it may even prevent stylization from improving the mechanical structure by accident. For novice modelers, this likely requires them to use open-source models and trust that they meet their needs or fabricate the original model to test out before stylization. 

This also limits MechStyle's ability to integrate with recent Generative AI-based methods that allow text-based generation of 3D models without an original model. These systems generate models solely based on aesthetic criteria and the results are unlikely to satisfy mechanical constraints. If these are used as inputs to MechStyle, it would likely preserve broken models that do not function in the real world. To extend our approach to 3D generation, the challenge is to predict a model's structural attributes during its generation. One approach to consider in future work is to predict mechanical properties based on datasets of fabricated 3D models, rather than requiring an already working model apriori.

\subsection{Preserving Multiple Mechanical Properties}
We assume that stress/strain simulations will reveal the parts of a model that must be preserved to ensure it is mechanically viable after stylization. However, these simulations only account for a small subset of mechanical constraints placed on a model. Finite Element Analysis is an effective simulation strategy that relies only on model geometry and a specified model material. However, other mechanical failures can result from complex relationships between geometry, fabrication method and setting (e.g., Slicer setting), and load conditions. While in a traditional CAD pipeline, an expert user may be able to specify each of these features, a novice maker is unlikely to correctly define the use case of their model. Alternatively, we could imagine a system that simulates these real-world conditions and materials but this poses several non-trivial challenges, including estimating material stiffness,  sim-to-real gap~\cite{wang2024diffusebot}, etc. This would require studies on more high-fidelity physics-based simulation. Fortunately, MechStyle does not rely on the specific implementation of mechanical simulation. While we use an existing FEA implementation, improved and customized simulations can be plugged into the system.

\subsection{Generalization of Simulation Scenarios}
MechStyle uses a model-agnostic mechanical simulation method, specifically a `drop-test', to assess structural integrity. While effective for a broad overview, this method may not capture the nuanced mechanical responses specific to different models under specific conditions. In a traditional CAD pipeline, a technical expert will manually specify more accurate boundary conditions for an accurate FEA simulation. Making this specification task accessible to novices would require new methods to extract implicit constraints from usage data. For example, we could imagine a system that models boundary conditions based on a video of the modeler using the original model for a specific activity. In place of the general-purpose drop-test, MechStyle could readily accept a use-case-specific simulation defined by such novice-oriented interactions. 

% \section{Limitations}
% \subsection{Predicting Fracture of Stylized 3D Models}
% In this work, we do not predict when a stylized version of a 3D model will fail post-fabrication. This is due to three significant factors: Firstly, 3D models are traditionally simulated under model-specific and usage-specific loading conditions, and the results are analyzed to find specific scenarios that would lead to a fracture of a 3D model. Secondly, the structural properties of a 3D model are heavily dependent on the fabrication method, the processing (slicing) settings, etc, that are not captured in simulation. Finally, we assume that the original model loaded by the user is structurally valid, and will be functional post-fabrication. We modify the stylization process to have minimal impact on the structural integrity (as informed by the original model) while maximizing the structural integrity of the model. Future work can extend this work by creating a ground-truth dataset of objects and their specific yield scenarios. By leveraging this dataset, we would be able to predict potential fractures in 3D models, allowing for a wider range of stylization. 

% \subsection{Limits of Performance Analysis}
% Another limitation is the gap between simulated results and fabricated model properties. While the hardware experiments presented in this paper show a proof-of-concept of how mechanical simulations can be used to generate structurally viable models, 

% % \subsection{Focus on Single-Component Models}
% % MechStyle currently only supports simulating single-component-based 3D models - models that do not require assembly post-fabrication. Extending to multi-component-based 3D models requires predicting the assembly steps, to allow for an accurate simulation. Future work can focus on integrating automated assembly tools, such as ASAP~\cite{tian2023asap} into MechStyle, which will enable this tool to support multi-component-based stylization. 

% % \faraz{Add the point that the user can test the individual parts, and test for their structural validity. The combination (assembly) might have different issues, and we can focus on them next. }

% \section{Discussion}

% Generative AI is allowing people to recreate and change models for fabrication, but they may not have the actual technical training on how to do it. This paper allows   


% The scarcity of well-annotated, fabrication-centric datasets represents a significant gap, but also an exciting opportunity, in the realm of 3D model customization. As the practice of digital fabrication continues to diversify and expand—evidenced by the growing variety of models and the emergence of specialized sub-domains like healthcare 3D printing—there is an increasing need for comprehensive datasets that go beyond geometry.

% % \subsection{Predicting Stress Distributions for Modified Geometry}
% % One primary challenge for MechStyle is its requirement for repeated computationally expensive simulations to estimate local stress values. While our current method incorporates adaptive strategies to schedule simulations efficiently, future work can focus on developing a predictive model that estimates the per-element stresses without an explicit simulation. This approach would involve the creation of a comprehensive dataset that correlates specific geometrical configurations of 3D models with their corresponding local stress outcomes. Leveraging such a dataset, a deep-learning network could be trained to predict stress values based on modifications in local geometry. By enabling real-time stress estimation at every iteration, such a model would facilitate a more dynamic adaptation of the stylization process, ensuring that structural integrity is maintained without the overhead of continuous simulation.

% \subsection{Model-Specific Simulations with Predictive Boundary Conditions}


% % \faraz{The people who will be using this tool do not know how to FEA simulation. The user can't specify the loading condition, so the problem was to find a way to simulate without asking the user to give them. Next, we can make solutions that infer conditions from usage, such as video of the original model in use. }
% % In the future, we will explore predicting model-specific boundary conditions for a more accurate simulation. By creating a dataset that associates 

% \subsection{Structural Analysis in 3D Generative AI}









% \subsection{Opportunities with Extended Datasets}


% Since we are using the simulation to evaluate 3D printed models, it was shown that using a hyperelastic material model is needed for PLA and that the Neo-Hookean model had a fairly good agreement with the experimental data [cite this paper: Nonlinear Material Modeling for Mechanical Characterization of 3-D Printed PLA Polymer With Different Infill Densities].


% There are several opportunities to curate or generate functionality information for 3D models. Although makers frequently upload 3D models, these are often not accompanied by detailed source files or annotations that could facilitate functional analysis. Encouraging the sharing of well-documented source files represents a cultural shift within these communities but has the potential to dramatically enrich the available datasets. Such a change would make these platforms more valuable as learning and experimentation spaces, aligning with the user-education focus often seen in HCI research. This is evident in newer sub-domains of making, where models are shared with additional labels (e.g., clinical reviews on the NIH 3D print exchange). 

% Extending datasets to include structural analysis parameters like loading conditions can offer another layer of functionality. By teaching machine learning algorithms to understand these relationships, we can pave the way for systems that not only allow for aesthetic customization but also offer models that are mechanically sound and functional in real-world conditions.

==> Sections/11_acknowledgements.tex <==

% \changes{
\begin{acks}
% \section{Acknowledgments}

\changes{
We would like to extend our sincere gratitude to the MIT-Google Program for Computing Innovation for their generous support, which made this research possible. Furthermore, we thank Varun Jampani, Yingtao Tian, Vrushank Phadnis, Yuanzhen Li, and Douglas Eck from Google for their valuable insights and feedback on this research.     
}
\end{acks}

% }

==> Sections/implementation.tex <==
\subsection{Simulation Issues}
\textbf{Talk about Semi-Implicit Euler method,} and the requirement to find an efficient delta\_t value. This is important, because too small a value will lead to a very slow simulation, and too large a value will lead to numerical instability. This value changes because stylized models have different geometry, and hence a different delta\_t for their analysis. Before running all the simulations for this, we run binary search for sim\_dt values over a range of values to search for an efficient number that creates a stable simulation, and run that. 

\textbf{Tetrahedralization}: Requires a fast, and efficient method, maximizing the quality while reducing the impact on the speed. 

\textbf{Matching vertices between tetrahedral file and the original mesh:} The OBJ and TET file are different because TET is a volumetric file. We match the vertex by finding an intersection of points from the TET file to the OBJ file, and then propagate the gradients accordingly. 

\subsection{Simulation Issues}
\textbf{Talk about Semi-Implicit Euler method,} and the requirement to find an efficient delta\_t value. This is important, because too small a value will lead to a very slow simulation, and too large a value will lead to numerical instability. This value changes because stylized models have different geometry, and hence a different delta\_t for their analysis. Before running all the simulations for this, we run binary search for sim\_dt values over a range of values to search for an efficient number that creates a stable simulation, and run that. 

\textbf{Tetrahedralization}: Requires a fast, and efficient method, maximizing the quality while reducing the impact on the speed. 

\textbf{Matching vertices between tetrahedral file and the original mesh:} The OBJ and TET file are different because TET is a volumetric file. We match the vertex by finding an intersection of points from the TET file to the OBJ file, and then propagate the gradients accordingly. 



==> Sections/notes.tex <==
ection{What are we doing here?}
For Style2Fab, we manipulated an existing 3D model to ascribe to a particular aesthetic style of the user. Since a 3D model can have multiple functional and aesthetic segments, we first segment the model and preserve the geometric aspects of this model to preserve the overall intended functionality. 

However, we realized that when we manipulate the geometry of the 3D model to get the intended texture of the user, we also affect the physical characteristics of the 3D model. For example, when we manipulated the texture of the splint design to have a blue-kintted texture, we got the desired rough texture, but we also made the model significantly weaker. This leads to the question: Can we use this technique to extend the user's control for physical properties as well? 

Few ideas for the interaction: 

Instead of finding a global level of physical capability (how strong, flexible a model is), we can keep the results relative to the original model. So, when the user first applies the texture to a 3D model, the system will annotate the 3D model to not just show the color and texture, but also give relative strength properties. For example, when the splint design would be highlighted, it will show that the stress / displacement thresholds are 40\% of the original design. Next, the user can use the slider for different properties to control -  for example flexibility, strength etc.  This control can be on the segment level, as well as entire 3D model level. This would require a multi-goal optimization, meaning there will be 2 networks: the Text2Mesh network that manipulates the 3D model for a specific texture, the new property control network that analyzes the physical properties and gives a heatmap. We combine the gradient and send back the results to the interface.  

- Another possible method is to allow a Pareto-Optimal space exploration. Since the stylization and FEA results might have different directional gradients, we can sample that space, and show multiple results that work for a user. Using the thumb splint as an example again: the system could show multiple results: 1) best combination of texture + rigidity 2) flexible 3) flexible on the hand segment + texture 4) best flexibility 5) best texture. The user can now either use one of these results directly, or use one of them as intermediate results, and fine-tune. 

\section{Questions}
\begin{enumerate}
    \item Are we manipulating the model's geometry, or are we changing the 3D printing material to be used for that part? 
    Both approaches have pros and cons. The pros of this approach is that it gives us a good story with the aesthetical property being changed with Style2Fab, and then we have the functional property being manipulated with the geometry as well. The con maybe that the ranges allowed would be limited by the material used. The way we can control this is that we can have an ML network recommend the material to use given the stress and strain regions of the model. This would work well with the J55 printer as well. 

    \item Where are getting the data from ? 
    Design and fabrication of materials with desired deformation behavior (https://dl.acm.org/doi/10.1145/1833349.1778800). This paper talks about collection of a dataset of deformation of 3D printed objects, and then using it as a library to combine internal structures of the model giving certain flexibility properties. 

    \item What are the different properties that we let the user control? 

    \item Can the system give recommendations on printing a model with specific materials as well, given the FEA results ? For example, a 3D model that has high displacement values, and low stress thresholds should be printed with certain flexible materials. 

\end{enumerate}
    



Useful phrases: 
As humans, we regularly link shape of an object with its built material. But in the context of geometric modeling, this inter-relation between form and material is rarely explored. 

\subsection{Experiments}
\paragraph{How much does the FEA result change when we use Text2Mesh on a model? Does it vary across prompts?:}

We sample 100 3D models from a Thingiverse dataset, and stylize them. We get the FEA analysis done both before and after stylization. We applied a variety of different textures: \faraz{What are these textures?} We found that the on average, XX property changed by YY, \faraz{Make a table. }

This means the following. 

\paragraph{Can we use FEA results as gradients to improve specific physical properties?: }

\paragraph{Can the FEA results be used in combination with the gradients from Text2Mesh?: }

\paragraph{Can we create a Pareto Optimal Space here, and sample points here to get models with those properties?: }

Amira: This is a question that people are still exploring. There are multiple approaches for it - for example: controlling the global properties by making local changes. 
Two approaches: Morphing the geometry

\paragraph{How do we define flexibility, and these properties? }
Flexibility == compliance. 
Maximum compliance doesn't make sense. 
If we keep the volume of the material between the models to be the same, then we can compare the compliance. 

There are ways to keep the same volume but increase or decrease the compliance. 

The model needs to be remeshed to have tetrahedrals instead of the tri-meshes. 

Get gradSim to work on a machine and let Amira know. Try out gradSim as a replacement for FEA. Think about an argument why it would make sense to have that instead of FEA, or maybe some combination. 
Particle systems are easier to simulate. 


==> useful_text.tex <==

Stochastic Structural Analysis for Context-Aware Design and Fabrication

The primary computational technique for failure analysis of solid structures is the finite element method [Belytschko et al. 2013], which allows for large-scale analysis of complicated structures and materials.  Of particular interest to us are so-called “worst-case” methods [Stava et al. 2012;  Zhou et al. 2013] which attempt to identify the most flimsy parts of a design so that users can modify them. These methods suffer from at least one of two fundamental limitations.  The first is that presenting mechanical stress, or arbi- trary, spatially varying weakness ratings to a designer is nonintuitive. Without further understanding of structural mechanics, the designer cannot reliably interpret how often these stresses/weak components will lead to breakage. This means the designer cannot fully under- stand whether he should compromise the aesthetic of the object in search of reliability. Second, the “worst-case” scenario, the one in which the object fails most easily, may never be encountered during real-world usage of the object. Thus, designing to account for these can lead to ‘over-engineering’ that costs time and money, and can sacrifice the design aesthetics.


Stress Relief: Improving Structural Strength of 3D Printable Objects

The promise of seamlessly moving creations from a virtual space into reality is truly tantalizing, and its applications go far beyond basic manufacturing and rapid prototyping.   Unfortunately,  many obstacles remain for 3D printing to be practical and commonplace. Although the quality of 3D printing has increased, both the time to print and the material costs have remained high. For a model to be 3D printable, it must meet a set of topological requirements to en- sure that its interior and exterior volumes are clearly defined.  This is usually achieved by making the input mesh a watertight manifold surface. Producing watertight manifold models from, for example, point clouds or surface representations has been well studied and is available in existing systems [Hornung and Kobbelt 2006; Liu et al. 2007].   Another  common  requirement  is  that  the  input  mesh  has no parts thinner than the printer can print.  However, these require- ments do not reflect the structural stability of the model. The man- ufactured objects are commonly so fragile that they do not survive transportation,  cannot  be  handled,  and  even  collapse  under  their own weight.

Furthermore, this work does not address the funda-
mental goal of correcting the detected structural issues. Even in the presence of perfect analysis, it may not be obvious or easy for the user to know where to start making corrections.  In our work, we underscore the importance of having both computer-assisted cor- rection and detection combined in a tightly coupled system.

We propose a first step in the direction of physically based auto- matic solutions for the detection and correction of major structural problems in 3D models before they are printed, while attempting to minimally alter their appearance as shown in Fig. 1.   We first detect major printability issues of the input model through print- ability assessments.  In our work, we focus on structural problems resulting from forces that can occur when the object is standing or when it is held at probable locations, such as pedestals or appro- priately sized handles.  We then correct the model by using three different approaches: local thickening, strut adding, and hollowing. Local thickening increases the strength of the object’s thin parts, and it preserves the form and the surface detail of the object. Struts can be inserted to prevent nonrigid deformations of the object, and they are automatically placed at locations that are least visible to the user. Hollowing eliminates material inside the object, reducing the weight of certain parts to alleviate the stress at other locations. Hollowing may also lower the cost by reducing the amount of used material.  The correction technique is chosen based on the visual impact on the result, and it can be further adjusted by user parame- ters.  After a correction is made, the process repeats until all struc- tural problems are eliminated.  We show our technique on various objects, such as game characters or technical models. We measured the stress on original and corrected objects, and we experimentally verified that the corrected models are more robust.  Our paper con- tinues  with  a  description  of  the  overall  schema  of  the  system  in Section 2.
